Conditional Generative Adversarial Networks for Optimal Path Planning

Path planning plays an important role in autonomous robot systems. Effective understanding of the surrounding environment and efficient generation of optimal collision-free path are both critical parts for solving path planning problem. Although conventional sampling-based algorithms, such as the rapidly-exploring random tree (RRT) and its improved optimal version (RRT*), have been widely used in path planning problems because of their ability to find a feasible path in even complex environments, they fail to find an optimal path efficiently. To solve this problem and satisfy the two aforementioned requirements, we propose a novel learning-based path planning algorithm which consists of a novel generative model based on the conditional generative adversarial networks (CGAN) and a modified RRT* algorithm (denoted by CGANRRT*). Given the map information, our CGAN model can generate an efficient possibility distribution of feasible paths, which can be utilized by the CGAN-RRT* algorithm to find the optimal path with a non-uniform sampling strategy. The CGAN model is trained by learning from ground truth maps, each of which is generated by putting all the results of executing RRT algorithm 50 times on one raw map. We demonstrate the efficient performance of this CGAN model by testing it on two groups of maps and comparing CGAN-RRT* algorithm with conventional RRT* algorithm.

==> sections/case_study.tex <==
In this section, we first illustrate the objective of our conditional GAN model in Sections IV-A.
Then the structure and loss function of the generator and discriminator is present in Sections IV-B and IV-C. 
Finally, we introduce the CGAN-RRT* procedure in Sections IV-D.

\begin{figure*}
	\centering
	\includegraphics[width=1\linewidth]{Figure/network_model}
	\caption{}
	\label{fig:f3}
\end{figure*}

\subsection{Objective}
Usually, the Generative Adversarial networks (GANs) are designed to learn a mapping from random noise $z$ to the objective output image $y$.
Then We have $\{G:z \rightarrow y\}$, where $G$ represents the generator of a GAN.
It is trained to generate output images that can confuse the discriminator, $D$. 
$D$ is trained to distinguish the $fake$ images produced by $G$ from the $real$ images with ground truth data.
In this problem, as shown in figure 3, the $fake$ images represent the images with paths generated by the generator, while the $real$ images represent the images with ground truth paths obtained from the RRT algorithm. 
The objective of a GAN can be expressed as:
\begin{equation}\label{key}
\begin{aligned}
\mathcal{L}_{GAN}(G,D) = & \mathbb{E}_{y}[logD(y)] +
\\ 
& \mathbb{E}_{x,z}[log(1-D(G(x,z))].
\end{aligned}
\end{equation}
The generator is trained to minimize the objective, while the discriminator is trained to maximize it. 
Then the problem of an unconditional GAN is represented as $\theta^{*} = \mathrm{arg \,min_{G} max_{D}}\mathcal{L}_{GAN}(G,D)$.


In contrast to the unconditional GAN, the conditional-GAN learns a mapping from observed image $x$ and random noise $z$ to output image $y$.
As the discriminator observes $x$, the objective function of the conditional-GAN is expressed as:
\begin{equation}\label{key}
\begin{aligned}
\mathcal{L}_{cGAN}(G,D) = & \mathbb{E}_{x,y}[logD(x,y)] +
\\ 
& \mathbb{E}_{x,z}[log(1-D(x,G(x,z))].
\end{aligned}
\end{equation}

We add L1 loss to encourage less blurring, which is the mean absolute error between the generated image and the target image.
Then the final objective of our conditional-GAN model is represented as $\theta^{*} = \mathrm{arg \,min_{G} max_{D}}\mathcal{L}_{cGAN}(G,D) + \lambda\mathcal{L}_{L1}(G)$,
where $\lambda$ is decided by us. In this article, we set $\lambda=100$.

%\begin{figure}
%	\centering
%	\includegraphics[width=1\linewidth, height=0.17\textheight]{Figure/simple_network}
%	\caption{}
%	\label{fig:simplenetwork}
%\end{figure}

\subsection{Generator architectures}
For the path generation problem, we aim to translation a high resolution input image to another high output image. 
Both corresponding input and output image share the same basic structure - raw map without paths. 
They just differ in surface where the output image has generated paths on map.
Our generator architecture is designed under this consideration.
Our proposed model is shown in fig. 4.
All convolutions are 4*4 spatial filters applied with stride 2.
Convolutions downsample by a factor of 2 in the encoder and upsample by a factor of 2 in the decoder.
The input of generator are raw images without paths, which have a dimension (256,256,3).
It means that they are pictures of 256*256 size with 3 channels.


For the encoding stage, we use modules of the form convolution-Batchnorm-ReLU.
The output of every encoding layer is called feature map. 
Low convolutional layers extract low-level feature maps and they are fed into a higher convolution layer to extract a high-level feature map.
If we denote each encoding layer with k filters as $\mathit{C_{k}}$, the encoder architecture can be expressed as:
$\mathit{C_{64}}$-$\mathit{C_{128}}$-$\mathit{C_{256}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$.
The Batchnorm layer aims to perform the normalization operation for each training mini-batch.  
It can accelerate the neural network training process and deal with the problem of parameter initialization. [1]
The rectified linear unit (ReLU) activation layer is widely used in neural network, which can help avoid the over-fitting problem.
It assigns zero output for negative input.
The activation function of it is defined as $f(x)=max(0,x)$, where $x$ is the input value.
Leaky-ReLU is a variant of ReLU. 
It translates negative input into output in the range of (0,1), that is $f(x)=max(\alpha x,x)$.
All ReLU activation layers in the encoder are leaky, with slope $\alpha=0.2$.



For the decoding stage, we use modules of the form convolution-Batchnorm-dropout-ReLU.
Let $\mathit{CD_{k}}$ denote the decoding layers with a dropout rate of 50\%, then the decoder architecture can be expressed as:
$\mathit{CD_{512}}$-$\mathit{CD_{512}}$-$\mathit{CD_{512}}$-$\mathit{C_{512}}$-$\mathit{C_{256}}$-$\mathit{C_{128}}$-$\mathit{C_{64}}$.
For a number of conditional-GAN models, random noise $z$ is added into the input of generator to avoid generating deterministic outputs.
However, the generator tend to ignore the random noise, which make this strategy ineffective.
In our decoder architecture, dropout layer is utilized to act as noise and ensure randomness, which randomly sets a half of input units to zero at each step. 
We apply the dropout layer in the first three decoding layers at both training and test time.
All ReLUs in the decoding stage is not leaky.


We adapt ``U-NET'' as the backbone of our generator network decoder. 
It is designed for shuttling abundant information between the input and output directly across the network.
In the generator architecture, we have $n$ layers. 
``U-NET'' is utilized by adding skip connections between each layer $i$ and layer $n-i$, simply concatenating all channels of them respectively.
Then the number of channels in decoder is changed, and the final decoder architecture can be expressed as:
$\mathit{CD_{512}}$-$\mathit{CD_{1024}}$-$\mathit{CD_{1024}}$-$\mathit{C_{1024}}$-$\mathit{C_{1024}}$-$\mathit{C_{512}}$-$\mathit{C_{256}}$-$\mathit{C_{128}}$.
The last layer in decoder is followed by a convolution layer and a Tanh activation function. Then the generator will output images with generated paths.


As generator is trained to produce images that cannot be distinguished from ground truth images, we define the generator loss as a sigmoid cross entropy loss of the generated images and an array of ones. The L1 loss is added for reducing blurring. Then the loss function of generator is shown as follows:
\begin{equation}\label{key}
\mathit{L_{G}} = sce(G(x),1)  +\lambda\mathcal{L}_{L1}(G),
\end{equation}
where $\lambda=100$.
\subsection{Discriminator architectures}
The discriminator architecture includes two pairs of input. 
One pair is the input map and the ground truth image, which should be classified as real.
Another pair is the the input map and the generated image produced by the generator, which should be classified as fake.
We concatenate each pair and perform encoding procedure respectively, using modules of the form convolution-Batchnorm-ReLU.
Then the architecture can be expressed as:
$\mathit{C_{64}}$-$\mathit{C_{128}}$-$\mathit{C_{256}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$-$\mathit{C_{512}}$.
All ReLU activation layers in the architecture are leaky, with slope $\alpha=0.2$.
The last layer is a one-dimensional output, followed by a Sigmoid function.


As discriminator is trained to distinguish output images produced by generator from target images, we define the discriminator loss as the sum of real loss and generated loss. 
Real loss is a sigmoid cross entropy loss of the ground truth images and an array of ones and generated loss is a sigmoid cross entropy loss of the generated images and an array of zeros, respectively. 
Then the loss function of discriminator is shown as follows:
\begin{equation}\label{key}
\mathit{L_{D}} = sce(G(x),0)  + sce(y,1).
\end{equation}
The generation procedure of ground truth images $y$ is described in Section V.

\subsection{CGAN-RRT*}
\begin{algorithm}[h]
	\normalsize
	\label{RRT}
	\caption{The CGAN-RRT* Algorithm}
	$V$ $\gets$ \{$x_{init}$\}; $E$ $\gets$ $\emptyset$;
	\\
	$\mathcal{P} \gets \mathrm{CGANModel}(Map,y)$;
	\\
	\For {$i$=1,. . .,$n$}{
		\eIf{$Rand() \textless 0.5$}
		{$x_{rand} \gets \texttt{Nonuniform($\mathcal{P}$)}$}
		{$x_{rand} \gets \texttt{Samplefree}_{i}$}
		{$x_{nearest}$} $\gets$ \texttt{Nearest}($G=(V,E)$,{$x_{rand}$});
		\\
		{$x_{new}$} $\gets$ \texttt{Steer}({$x_{nearest}$},{$x_{rand}$});
		\\
		\If{$\texttt{ObstacleFree}({x_{nearest}},{x_{new}})$}
		{$V$ $\gets$ $V$ $\cup$ \{{$x_{new}$}\}; 
		\\
		$E$ $\gets$ $E$ $\cup$ \{{($x_{nearest}$,$x_{new}$)}\};
		\\
		Rewire();
		\\
		
		}
	}
	\textbf{Return} ($G=(V,E)$)
\end{algorithm}
The CGAN-RRT* algorithm differs from the traditional RRT* in sampling technique.
Thus, it can be applied to other sampling-based algorithms in the future research.
It utilizes the pre-trained conditional-GAN model to guide the sampling process of the RRT* algorithm.
There are two sampling ways in the CGAN-RRT* algorithm.
One is the nonuniform sampling way from the conditional-GAN model,
and another is the uniform sampling way from the conventional RRT* algorithm.


The details of the CGAN-RRT* algorithm is present in Algorithm 2. 
It is initialized with the initial state $x_{init}$ and no edges.
$\mathbf{CGANModel}(Map,y)$ produces the predicted sampling distribution $\mathcal{P}$.
At each iteration, a random number $\mathbf{Rand}() \in (0,1)$ is utilized to determine which sampling ways to choose.
If $\mathbf{Rand}() \textless 0.5$, a point $x_{rand} \in \texttt{Nonuniform($\mathcal{P}$)}$ is sampled.
Otherwise, the uniform sampling way is utilized.
Then the algorithm attempts to find the nearest vertex $v \in V$ to the new sample and connect them.
If there are no obstacles through the connection, $x_{new}$ is added to the vertex set $V$,
and ($x_{nearest},x_{new}$) is added to the edge set $E$.
The procedure of $Rewire$ enables the local path to converge to the global optimal path.
Finally, the CGAN-RRT* algorithm returns a graph of new vertex set $V$ and edge set $E$.




